Qompose: A Technique to Select Optimal Algorithm- Specific Layout for Neutral Atom Quantum Architectures

As quantum computing architecture matures, it is important to investigate new technologies that lend unique advantages. In this work, we propose, Qompose, a neutral atom quantum computing framework for efficiently composing quantum circuits on 2-D topologies of neutral atoms. Qompose selects an efficient topology for any given circuit in order to optimize for length of execution through efficient parallelism and for overall fidelity. our extensive evaluation demonstrates the Qompose is effective for a large collection of randomly-generated quantum circuits and a range of real-world benchmarks including VQE, ISING, and QAOA.

==> sections/related_works.tex <==
\section{Related Work and Conclusion}

Many works have been put forward in the way of superconducting quantum computing, while the pool of research in neutral atom quantum computing is more limited. Notably, \cite{baker2021exploiting} has laid the foundation for this work by providing a basis for mapping and routing for neutral atom circuits. Other works have provided thorough review into neutral atom quantum computing \cite{weiss2017quantum, henriet2020quantum,saffman2016quantum} which explain the procedures which we build out simulator on.  Additionally, \cite{li2019tackling,wille2019mapping} have tackled a similar mapping problem for qubit swaps, although these works focus on the space of superconducting hardware and not on neutral atom hardware. Recently, \cite{patel2023graphine} has proposed a technique to design application specific topologies for neutral atom circuits.

